Feasibility and Transferability of Transfer Learning: A Mathematical Framework

Transfer learning is an emerging and popular paradigm for utilizing existing knowledge from previous learning tasks to improve the performance of new ones. Despite its numerous empirical successes, theoretical analysis for transfer learning is limited. In this paper we build for the first time, to the best of our knowledge, a mathematical framework for the general procedure of transfer learning. Our unique reformulation of transfer learning as an optimization problem allows for the first time, analysis of its feasibility. Additionally, we propose a novel concept of transfer risk to evaluate transferability of transfer learning. Our numerical studies using the Office-31 dataset demonstrate the potential and benefits of incorporating transfer risk in the evaluation of transfer learning performance.

==> finance_alpha.tex <==
\section{Transfer Learning with Application in Stock Return Prediction}\label{sec:return_predict}

In this section, we consider  transfer learning for the stock return prediction problem, under the mathematical framework  proposed in the paper. Numerical experiments will show the consistency of the transfer risk with classical statistical metrics. In addition, improved prediction accuracy may be achieved under appropriate  transfer learning over  direct learning. 

\subsection{Prediction problem and setup}\label{sec:return_predict_set_up}
The task is to predict a stock's daily return based on its historical daily return and daily trading volume data.

\paragraph{Data pre-processing via signature transform.}
Denote $\{s_\tau\}_{\tau\geq 0}$ as the historical daily close price of a stock and $\{v_\tau\}_{\tau\geq 0}$ as its historical daily trading volume. To facilitate the subsequent computation, we first apply the log transform to the data, which results in $\{\log(s_\tau)\}_{\tau\geq 0}$ and $\{\log(v_\tau)\}_{\tau\geq 0}$. At each time step $t=0, 1,\dots$, we aim to predict the next daily log return $y_t=\log(s_{t+1})-\log(s_t)$, based on the historical price and volume data $\{\log(s_\tau)\}_{0\leq\tau\leq t}$ and $\{\log(v_\tau)\}_{0\leq\tau\leq t}$.

To adopt  the transfer learning framework, we propose to generate  features from the data via the so called \textit{signature transform}, as recalled below.  
\begin{defn}[Signature]\label{defn:signature}
    For a continuous piecewise smooth path $x:[0,T]\to\R^d$, its signature is given by
    \[S(x)=(1,S(x)^{(1)},\dots,S(x)^{(n)},S(x)^{(1,1)},\dots,S(x)^{(i,j)},\dots,S(x)^{(n,n)},\dots),\]
    where for $m=1,2,\dots,$ and $i_1,\dots,i_m\in[n]$,
    \[S(x)^{(i_1,\dots,i_m)}=\int_{0\leq t_1<\dots<t_m\leq T}dx^{i_1}_{t_1}\dots dx^{i_m}_{t_m}.\]
    The truncated signature up to degree $M$ is given by
    \[S_M(x)=(1,S(x)^{(1)},\dots,S(x)^{(\overbrace{n,\dots,n}^{M})}).\]
\end{defn}
It is well known now that the signature of a path generated by a sequence of data essentially determines the path in a computationally  efficient way. Furthermore, its universal nonlinearity property allows for the approximation of  every continuous function of the path  by a linear function of its signature transform. 
Here in the prediction problem,  the features are constructed by the signature transform through the following procedure:
\begin{enumerate}
    \item Fix a time lag $L$ and an order parameter $M$.
    
    \item For each time step $t=0, 1,\dots$, consider the historical price and volume data with time lag $L$: $\{\log(s_\tau)\}_{t-L+1\leq\tau\leq t}$ and $\{\log(v_\tau)\}_{t-L+1\leq\tau\leq t}$.

    \item Consider a three-dimensional path $z_\tau=(\tau, \log(s_\tau), \log(v_\tau))$ for $t-L+1\leq\tau\leq t$, and compute its $M^{\text{th}}$-order truncated signature $x_t=S_M(z)$, as defined in Definition \ref{defn:signature}.

    \item Construct the data set for the prediction problem with the feature vector $x_t$ and the target variable $y_t$: $\{(x_t, y_t)\}_{t\geq 0}$. Each feature, as well as the target variable, will be standardized before inputting into any prediction model.
\end{enumerate}
The time lag parameter $L$ and the order parameter $M$ are the hyper-parameters of the prediction model, and their effects on the prediction accuracy will be studied in the numerical results.

\paragraph{Prediction with Ridge regression via direct learning.} Given the training set $\{(x_t, y_t)\}_{0\leq t\leq T-1}$, and in particular the universal non-linearity property of the signtuare transform, it is natural to consider a linear model $y_t=x_t\cdot\theta+\epsilon$  through the ridge regression. Here  the $L_2$ penalized  addresses the potential multi-collinearity issue of features from the signature transform. 

Given a particular target stock, a direct learning scheme  starts with constructing the signature feature data set $\{(x_t, y_t)\}_{0\leq t\leq T-1}$. Then the entire time horizon will be split into a training period and a testing period. A Ridge regression is then applied to fit the linear model on the train data set, and the performance of the model will be evaluated on the test data set.
More specifically, the Ridge regression finds the estimator $\widehat\theta$ by solving the following $L_2$ penalized least square problem 
\begin{align}\label{eqn:ridge}
\widehat{\theta}:=\argmin_\theta\frac{1}{T}\sum_{t=0}^{T-1}\left(x_t\cdot\theta - y_t\right)^2 + \lambda \left\|\theta\right\|_2^2.
\end{align}
The choice of the hyper-parameter $\lambda>0$ controls the bias-variance tradeoff of the method: a larger $\lambda$ indicates a lower variance while a higher bias.



Since the data set constructed from one single stock may only contain limited samples, it motivates the idea of boosting the prediction accuracy by transfer learning.

\paragraph{Prediction with Ridge regression via transfer learning.}
Transfer learning allows  one to first pre-train the Ridge regression model on a data set constructed from multiple stocks. That is, consider a target task which is to predict the return of one particular stock, say Apple. One can pre-train a model on a source task which contains several related stocks (such as Google, Amazon, Microsoft) from the similar industry. 
In order to transfer the per-trained model to the target task, one then again fits a new model with the Ridge regression, where the $L_2$ regularization term penalizes on the distance with respect to the pre-trained model.

Here the source task and target task share the same input and output spaces $\mathcal{X}_S=\mathcal{X}_T=\mathbb{R}^d_\text{sig}$ and $\mathcal{Y}_S=\mathcal{Y}_T=\mathbb{R}$, where $d_\text{sig}$ is the dimension of the signature feature and is fully determined by the order $M$. Meanwhile, the admissible sets of source and target models are restricted to all the linear functions from $\mathbb{R}^d_\text{sig}$ to $\mathbb{R}$: $A_S=A_T=\{f:\mathbb{R}^d_\text{sig}\to\mathbb{R}|f(x)=x\cdot\theta\text{ for some }\theta\in\mathbb{R}^d_\text{sig}\}$. Denote the source data set as $\{(x_{S,t}, y_{S,t})\}_{0\leq t\leq T_S-1}$ and the target data set $\{(x_{T,t}, y_{T,t})\}_{0\leq t\leq T_T-1}$. The pre-trained model is first obtained by solving the following optimization problem
\begin{align}\label{eqn:ridge_source}
\widehat{\theta_S}:=\argmin_\theta\frac{1}{T_S}\sum_{t=0}^{T_S-1}\left(x_{S,t}\cdot\theta - y_{S,t}\right)^2 + \lambda_S \left\|\theta\right\|_2^2.
\end{align}
This formulation \eqref{eqn:ridge_source} is equivalent to \eqref{eq: obj-s} by taking the loss function $L_S$ as the square loss plus a regularization term on the $l_2$-norm of the linear parameter $\theta$, while the expectation is taken over the empirical distribution of source samples $\{(x_{S,t}, y_{S,t})\}_{0\leq t\leq T_S-1}$.

Transfer learning is then to find the solution for the following optimization problem:
\begin{align}\label{eqn:ridge_target}
\widehat{\theta_T}:=\argmin_\theta\frac{1}{T_T}\sum_{t=0}^{T_T-1}\left(x_{T,t}\cdot\theta - y_{T,t}\right)^2 + \lambda_T \left\|\theta-\widehat{\theta_S}\right\|_2^2.
\end{align}
Here $\lambda_T>0$ in \eqref{eqn:ridge_target} is a hyper-parameter controls the power of the regularization: the higher $\lambda$ is, the closer the transferred model $\widehat{\theta_T}$ will be to the pre-trained model $\widehat{\theta_S}$. 

Note that from the point of view of \eqref{eq: doub-trans}, \eqref{eqn:ridge_target} is equivalent to searching an output transport mapping $T_Y$ over the linear function space $A_T=\{f:\mathbb{R}^d_\text{sig}\to\mathbb{R}|f(x)=x\cdot\theta\text{ for some }\theta\in\mathbb{R}^d_\text{sig}\}$, while the loss function $L_T$ takes the form of the square loss in addition to a regularization on the $l_2$ distance from the source model parameter $\widehat{\theta_S}$.

\subsection{Numerical results}
The data used in the  numerical experiment is the historical daily stock  price and trading volume from the Information Technology sector of the US equity market,  from February 2010 to September 2022. For each experiment, a set of eleven stocks will be first randomly sampled from the Information Technology sector, with the first ten of them served as the source task, and the last one as the target task. Three data sets will be constructed according to the data pre-processing steps discussed in Section \ref{sec:return_predict_set_up}:
\begin{enumerate}
    \item \textbf{Source training data}: which consists of the signature features and log returns of the first ten source stocks, from February 2010 to September 2021.

    \item \textbf{Target training data}: which consists of the signature features and log returns of the last target stock, from February 2010 to September 2021.

    \item \textbf{Target testing data}: which consists of the signature features and log returns of the last target stock, from September 2021 to September 2022.
\end{enumerate}

We compare two approaches
\begin{enumerate}
    \item \textbf{Direct learning}: the model is directly trained on the target training data by the ridge regression \eqref{eqn:ridge}.
    
    \item \textbf{Transfer learning}: the model is first pre-trained on the source training data by the ridge regression \eqref{eqn:ridge_source}, and is then retrofit on the target training data by \eqref{eqn:ridge_target}.
\end{enumerate}

The performances are evaluated on the target testing data through three different metrics: mean square error ($\textbf{MSE}$), $\textbf{R}^2$, and correlation between predicted return and actual return (\textbf{Corr}). We also change the hyper-parameters: lag $L$ and order $M$ in the signature-based feature generation steps to study their influences on the performances. The regularization parameters in \eqref{eqn:ridge_source} and \eqref{eqn:ridge_target} are set as $\lambda_S=1.0$ and $\lambda_T=5.0$. The full results are listed in Table \ref{tab:prediction}, and the results are averaged over two hundred random selections of stocks.

\begin{table}[H]
  \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \toprule
          & \textbf{Algorithm} & \multicolumn{3}{c|}{\textbf{Direct}} & \multicolumn{3}{c}{\textbf{Transfer}} \\
    \midrule
    \textbf{Lag} & \textbf{Order\textbackslash{}Metric} & \multicolumn{1}{c|}{\textbf{MSE}} & \multicolumn{1}{c|}{$\textbf{R}^2$} & \multicolumn{1}{c|}{\textbf{Corr}} & \multicolumn{1}{c|}{\textbf{MSE}} & \multicolumn{1}{c|}{$\textbf{R}^2$} & \multicolumn{1}{c}{\textbf{Corr}} \\
    \midrule
    \multirow{3}[6]{*}{\textbf{2.00}} & \textbf{2.00} & 1.21  & 0.07  & 0.03  & 1.66  & 0.08  & 0.04 \\
\cmidrule{2-8}          & \textbf{3.00} & 1.41  & 0.06  & 0.03  & \textcolor[rgb]{1,0,0}{1.15} & 0.07  & 0.03 \\
\cmidrule{2-8}          & \textbf{4.00} & 1.88  & -0.06 & 0.03  & 1.91  & 0.06  & 0.02 \\
    \midrule
    \multirow{3}[6]{*}{\textbf{3.00}} & \textbf{2.00} & 1.75  & 0.06  & -0.01 &  1.55  & 0.07  & -0.01 \\
\cmidrule{2-8}          & \textbf{3.00} & 1.58  & 0.04  & 0.02  & 1.27  & 0.05  & 0.03 \\
\cmidrule{2-8}          & \textbf{4.00} & 1.72  & -0.14 & 0.00  & 1.70  & -0.07 & 0.01 \\
    \midrule
    \multirow{3}[6]{*}{\textbf{5.00}} & \textbf{2.00} & 1.62  & 0.08  & 0.04  & 1.54  & \textcolor[rgb]{1,0,0}{0.08} & 0.06 \\
\cmidrule{2-8}          & \textbf{3.00} & 1.74  & 0.05  & 0.04  & 2.28  & 0.07  & 0.04 \\
\cmidrule{2-8}          & \textbf{4.00} & 1.63  & -0.13 & 0.02  & 2.05  & 0.05  & 0.06 \\
    \midrule
    \multirow{3}[6]{*}{\textbf{10.00}} & \textbf{2.00} & 1.31  & 0.08  & 0.06  & 1.75  & 0.08  & \textcolor[rgb]{1,0,0}{0.07} \\
\cmidrule{2-8}          & \textbf{3.00} & 1.45  & 0.04  & -0.01 & 1.53  & 0.07  & 0.04 \\
\cmidrule{2-8}          & \textbf{4.00} & 2.48  & -0.14 & 0.07  & 2.84  & -0.01 & 0.06 \\
    \bottomrule
    \bottomrule
    \end{tabular}
    \caption{Prediction performance of direct and transfer learning.}
  \label{tab:prediction}
\end{table}

\paragraph{Main findings.} In Table \ref{tab:prediction}, the top performer under each metric is marked red. For example, the lowest MSE is obtained when transfer learning  is applied to the prediction task, with $L=2, M=3$. As seen from the table,  transfer learning achieves the best results under all three different metrics, for this task of return prediction. 

Table \ref{tab:prediction_score} 
summarizes the relations between the Wasserstein-based transfer risk $\Ef^O_W(\widehat{\theta_S})$ in \eqref{eqn:W_risk}, where $p=2$, and three other standard metrics: MSE, $R^2$, and correlation. More specifically, with $L=5, M=2, \lambda_S=1.0, \lambda_T=5.0$, we randomly choose the source and target stocks as described earlier, apply transfer learning to the prediction problem under these four metrics. Here we record the negations of $\textbf{R}^2$ and $\text{Corr}$ so that lower numbers imply better performances. The correlation matrix, Table \ref{tab:prediction_score}, is computed over two hundred random experiments. It can be observed that the Wasserstein-based transfer gap is positively correlated with other three metrics, especially with the mean square error. This finding suggests that the lower the transfer risk, the better the transfer learning performance.

\begin{table}[H]
  \centering
    \begin{tabular}{c|cccc}
    \toprule
    \toprule
          & \multicolumn{1}{c}{\textbf{MSE}} & \multicolumn{1}{c}{$-\textbf{R}^2$} & \multicolumn{1}{c}{$-$\textbf{Corr}} & \multicolumn{1}{c}{\textbf{Transfer Risk}} \\
    \midrule
    \textbf{MSE} & 1.000 & 0.275 & 0.136 & 0.963 \\
    $-\textbf{R}^2$ & 0.275 & 1.000 & 0.588 & 0.401 \\
    $-$\textbf{Corr} & 0.136 & 0.588 & 1.000 & 0.173 \\
    \textbf{Transfer Risk} & 0.963 & 0.401 & 0.173 & 1.000\\
    \bottomrule
    \bottomrule
    \end{tabular}
  \caption{Correlation matrix of various metrics.}
  \label{tab:prediction_score}
\end{table}

Finally, it is worth pointing out  the impact of the signature order $M$: in most cases,  larger $M$ ($M\geq4$) does not improve the performance of either transfer learning or direct learning.    This implies that empirically, drift, volatility, and skewness (which correspond to signature features with $M\leq3$) are more useful in stock return predictions than other higher-order moments. And a large $M$, which may lead to an excessive number of features with possible over-fitting issues, is computationally expensive and unnecessary in the prediction task.


==> finance_portfolio.tex <==
\section{Transfer Learning with Application in Portfolio Optimization}\label{sec:finance_PO}
In this section, we will reinforce the connection between the performance of the transfer learning scheme \eqref{eq: doub-trans} and the transfer risk in \eqref{eqn:risk} through applying the transfer learning scheme to financial portfolio optimization. 

Throughout the experiments, we test the performance of transfer learning and transfer risk under various tasks, including cross-continent transfer (transferring a portfolio from the US equity market to the Brazil equity market), cross-sector transfer (transferring a portfolio from the technology sector to the health-care sector), and cross-frequency transfer (transferring a low-frequency portfolio to the mid-frequency domain). It is illustrated numerically that transfer risk is able to properly reflect the transferability of the optimization task, hence providing a computationally efficient way to identify suitable source tasks.


\subsection{Portfolio Optimization Problem Set-up}\label{subsec:port_opt_setup}
\paragraph{Portfolio Optimization Based on Sharpe Ratio.} Consider a capital market consisting of $d$ assets whose annualized returns are captured by the random vector $r = (r_1, ..., r_d)^\top \sim \mathbb{P}.$ A portfolio allocation vector $\phi = (\phi_1, ..., \phi_d)^\top$ is a $d$-dimensional vector in the unit simplex $\mathbb{X} := \{\phi \in \mathbb{R}^d_+: \sum_{j=1}^d \phi_j = 1 \}$ with $\phi_i$ percentage of the available capital invested in asset $i$ for each $i=1,...,d$. The annualized return of a portfolio $\phi$ is given by $\phi^\top r.$ 

We aim to find the optimal portfolio with the highest Sharpe ratio by solving the following optimization problem:    
\begin{equation}\label{eqn:portfolio_opt}
    \widehat{\phi}=\argmax_{\phi \in \mathbb{X}}\frac{\mathbb{E}^{\mathbb{P}}[\phi^\top r]}{\text{Var}(\phi^\top r)}=\argmax_{\phi \in \mathbb{X}}\frac{\mu_\mathbb{P}^\top\phi}{\phi^\top\Sigma_\mathbb{P}\phi},
\end{equation}
where $\mu_\mathbb{P}$ is the expectation and $\Sigma_\mathbb{P}$ is the covariance matrix  of the return $r$. Empirically, $\mu_\mathbb{P}$ and $\Sigma_\mathbb{P}$ are estimated from the historical return.

In many cases, such as managing portfolios in new emerging markets, there are limited data for directly estimating $\mu_\mathbb{P}$ and $\Sigma_\mathbb{P}$, which may result in large estimation error and lead to a non-robust portfolio. We will show here that transfer learning could be a natural and viable framework to resolve this problem.

\paragraph{Portfolio Optimization with Transfer Learning.} In this example, the source task and target task share the same input and output spaces $\mathcal{X}_S=\mathcal{X}_T=\mathbb{R}^d$ and $\mathcal{Y}_S=\mathcal{Y}_T=\mathbb{R}$, where $d$ is the number of assets in the portfolio. Note that different from the previous return prediction example, there is no sample from the output space that is explicitly observed. Instead, one can only get historical stock returns as input data. Meanwhile, a portfolio vector $\phi$ can be viewed as a linear mapping from $\mathbb{R}^d$ to $\mathbb{R}$, taking a $d$-dimensional stock return to a portfolio return. More specifically, the admissible sets of source and target models are restricted to: $A_S=A_T=\{f:\mathbb{R}^d\to\mathbb{R}|f(r)=\phi^\top r\text{ for some }\phi\in\mathbb{X}\}$. In addition, for the source task, the loss functional $\mathcal{L}_S$ in \eqref{eq: obj-s} is set to be the negative Sharpe ratio, and consequently, the source task is to solve following the optimization problem:
\begin{equation}\label{eqn:portfolio_opt_source}
    \widehat{\phi_S}=\argmax_{\phi \in \mathbb{X}}\frac{\mu_S^\top\phi}{\sqrt{\phi^\top\Sigma_S\phi}},
\end{equation}
where $\mu_S$ and $\Sigma_S$ are the mean and covariance estimations from the source data set. 

Then, the portfolio is transferred to the target task by solving the following optimization with a $L_2$ regularization term penalizing the distance between the pre-trained portfolio and the transferred portfolio:
\begin{equation}\label{eqn:portfolio_opt_target}
    \widehat{\phi_T}=\argmax_{\phi \in \mathbb{X}}\frac{\mu_T^\top\phi}{\sqrt{\phi^\top\Sigma_T\phi}}-\lambda\left\|\widehat{\phi_S}-\phi\right\|^2_2.
\end{equation}
Here $\mu_T$ and $\Sigma_T$ are the mean and covariance estimations from the target data, and $\lambda>0$ is a hyper-parameter controls the power of the regularization: the higher $\lambda$ is, the closer the transferred portfolio $\widehat{\phi_T}$ will be to the pre-trained portfolio $\widehat{\phi_S}$. From the point of view of \eqref{eq: doub-trans}, \eqref{eqn:portfolio_opt_target} is equivalent to searching an output transport mapping $T_Y$ over the linear function space $A_T=\{f:\mathbb{R}^d\to\mathbb{R}|f(r)=\phi^\top r\text{ for some }\phi\in\mathbb{X}\}$, while the loss functional $\mathcal{L}_T$ in \eqref{eq: doub-trans} takes the form of negative Sharpe ratio in addition to a regularization on the $l_2$ distance from the source model $\widehat{\phi_S}$.

There are three types of portfolio transfers considered in the experiments. 

\begin{enumerate}
    \item \textbf{Cross-continent transfer}: This refers to the case when one transfers a portfolio from the equity market in one country to the equity market in another country (e.g. from the US equity market to the Brazil equity market). In general, the source market has more historical data or more diverse stocks than the target market, which may provide the target market with a robust pre-trained portfolio. The study of cross-continent transfer aims to understand how continental discrepancy affects the performance of transfer learning. 

    \item \textbf{Cross-sector transfer}: This refers to the case when one transfers a portfolio from one sector of a market to another sector (e.g. from Information Technology sector to Health Care sector in the US equity market). The study of cross-sector transfer aims to understand correlations between various sectors in the market, and how correlations between sectors affect the performance of transfer learning.

    \item \textbf{Cross-frequency transfer}: This refers to the case when one transfers a portfolio constructed under one trading frequency to another trading frequency (e.g. from low-frequency trading to mid or high-frequency trading). The study of cross-frequency transfer aims to explore the possibility of transferring the portfolio across different trading frequencies, which has important and practical implications for institutional investors.
\end{enumerate}

\paragraph{Computation of Transfer risk.}
Different from the supervised learning setting, there is in general no output variable $y$ in the portfolio optimization problem. Hence, we propose the following approach to compute the transfer risk for portfolio optimization. Given the mean and covariance estimations for the source (resp. target) task, $\left(\mu_S, \Sigma_S\right)$ (resp. $\left(\mu_T, \Sigma_T\right)$), we approximate the return distribution in the source (resp. target) task by a multivariate normal distribution $\mathcal{N}\left(\mu_S, \Sigma_S\right)$ (resp. $\mathcal{N}\left(\mu_T, \Sigma_T\right)$). Then the (approximated) transfer risk is defined as the Wasserstein-2 distance between $\mathcal{N}\left(\mu_S, \Sigma_S\right)$ and $\mathcal{N}\left(\mu_T, \Sigma_T\right)$. This definition can be essentially viewed as computing the input transport risk for the identity input mapping $T_0^X=id_{\mathcal{X}}$.

\subsection{Numerical Results}

\paragraph{Cross-Continent Transfer.} 
In the numerical experiments, the source market is fixed to be the US equity market, while the target markets are chosen to be United Kingdom, Brazil, Germany, and Singapore, in four separate experiments.

Given a target market, we first select out the top ten stocks with the largest market capitals ($d=10$) as the class of target assets. Then, ten stocks will be randomly selected from the S\&P500 component stocks as the class of source assets. Three data sets will be constructed accordingly:
\begin{enumerate}
    \item \textbf{Source training data}: it consists of the daily returns of ten source assets, from February 2000 to February 2020.

    \item \textbf{Target training data}: it consists of the daily returns of ten target assets, from February 2015 to February 2020.

    \item \textbf{Target testing data}: it consists of the daily returns of ten target assets, from February 2020 to September 2021.
\end{enumerate}

We compare direct learning with transfer learning: for direct learning, the portfolio is directly learned by solving \eqref{eqn:portfolio_opt}, with mean and covariance estimated from target training data; for transfer learning, the portfolio is first pre-trained on the source training data by solving \eqref{eqn:portfolio_opt_source}, then fine-tuned on the target training data by solving \eqref{eqn:portfolio_opt_target}. Finally, the performances of those methods are evaluated through their Sharpe ratios on the target testing data. The regularization parameter $\lambda$ in \eqref{eqn:portfolio_opt_target} is set to be $0.2$. Meanwhile, we also compute the transfer risk following the method described in Section \ref{subsec:port_opt_setup}, using the source training data and target testing data.

For each target market, the results across one thousand random experiments (randomness in selections of source assets) are plotted in Figure \ref{fig:cross_continent}. 
%Note that the horizontal score'' axis represents the negation of the transfer score: a higher negative transfer score implies a better transferability between the source and target task.

Across those four markets, a consistent pattern is observed: the transfer risk is negatively correlated with the Sharpe ratio of the transferred portfolio (with correlation around -0.4). For example, the correlation is -0.42 when transferring to the UK market, and -0.44 when transferring to the Brazil market. This observation supports our idea of using transfer score as a measurement to the transferability of a task.

Meanwhile, the performance of transfer learning is compared with that of direct learning in Figure \ref{fig:cross_continent}. For each target market, the dashed green line indicates the direct learning performance. The blue dots above the green line represent transfer learning tasks that outperform the direct learning. Note that for all four target markets, there are a significant amount of transfer learning tasks outshining the direct learning, especially for those tasks achieving low transfer risk.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/US-UK.png}
         \caption{US$\to$UK, correlation=-0.40}
         \label{fig:US-UK}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/US-Brazil.png}
         \caption{US$\to$Brazil, correlation=-0.37}
         \label{fig:US-Brazil}
     \end{subfigure}
\end{figure}
\begin{figure}[H]\ContinuedFloat
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/US-Germany.png}
         \caption{US$\to$Germany, correlation=-0.41}
         \label{fig:US-Germany}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/US-Singapore.png}
         \caption{US$\to$Singapore, correlation=-0.34}
         \label{fig:US-Singapore}
     \end{subfigure}
     \caption{Sharpe ratio and transfer risk when transferring from the US market to other markets.}
     \label{fig:cross_continent}
\end{figure}

As shown in Figure \ref{fig:cross_continent}, transfer learning is more likely to outperform direct learning in European markets, such as UK and Germany, while it performs worse in the Brazil market. A possible interpretation to this finding is that European markets have tighter connections and higher similarities with the US market, which help to boost the performance of transfer learning.

\paragraph{Cross-Sector Transfer.} In the following numerical experiments, we focus on transfer learning between ten different sectors in the US equity market: Communication Services, Consumer Discretionary, Energy, Financials, Health Care, Industrials, Information Technology, Materials, Real Estate, Utilities.

Given a source sector and a target sector, we first randomly sample ten stocks ($d=10$) from each sector, as the source asset class and target asset class. Then, three data sets will be constructed accordingly:

\begin{enumerate}
    \item \textbf{Source training data}: it consists of the daily returns of ten stocks from a given source sector, from February 2000 to February 2020.

    \item \textbf{Target training data}: it consists of the daily returns of ten stocks from a given target sector, from February 2015 to February 2020.

    \item \textbf{Target testing data}: it consists of the daily returns of ten stocks from a given target sector, from February 2020 to September 2021.
\end{enumerate}

The transfer learning scheme applied in the experiments is same as before: the portfolio is first pre-trained on the source training data by solving \eqref{eqn:portfolio_opt_source}, then fine-tuned on the target training data by solving \eqref{eqn:portfolio_opt_target}. Finally, the performance of the portfolio is evaluated through its Sharpe ratio on the target testing data. The regularization parameter $\lambda$ in \eqref{eqn:portfolio_opt_target} is set to be $0.2$. Meanwhile, the computation of transfer risk follows the approach described in Section \ref{subsec:port_opt_setup}, using the source training data and target testing data. 

For each source-target sector pair (in total $10\times10=100$ pairs), five hundred random experiments with different stock selections are conducted, and we record the average Sharpe ratio and average transfer risk of those random experiments. The results are presented in Figure \ref{fig:sector_sp500_health}, Figure \ref{fig:cross_sector_sp500}, Figure \ref{fig:cross_sector_nonsp500} and Table \ref{tab:cross_sector_corr}. 
%Similar as Figure \ref{fig:cross_continent}, the term ``score'' in the following figures and tables refers to the negation of the transfer score: a higher ``score'' implies a higher similarity and better transferability between the source and target task.

Figure \ref{fig:sector_sp500_health} shows the relation between (average) Sharpe ratios and (average) scores when transferring portfolios from various source sectors to the target Health Care sector. In general, the negative correlation between Sharpe ratios and scores is observed: when the target sector is fixed (Health Care in this example), transferring a portfolio from a source sector with lower transfer risk is more likely to achieve a higher Sharpe ratio. In particular, Information Technology, Health Care, and Consumer Discretionary are desirable source sectors when the target sector is Health Care, while Energy is not a suitable choice.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/sector_sp500_health.png}
    \caption{Transfer risk and Sharpe ratio, transferring to Health Care sector in S\&P500 stocks.}
    \label{fig:sector_sp500_health}
\end{figure}

In Figure \ref{fig:cross_sector_sp500} and Figure \ref{fig:cross_sector_nonsp500}, we plot the heat maps of transfer risks and Sharpe ratios when transferring across all sectors. Here the transfer risks and Sharpe ratios are rescaled linearly so that for each target sector, the values will range from zero to one, where zero (resp. one) is for the source sector with the lowest (resp. highest) transfer risk or Sharpe ratio. Meanwhile, for experiments in Figure \ref{fig:cross_sector_sp500}, the source and target stocks are all sampled from S\&P500 components, while for Figure \ref{fig:cross_sector_nonsp500}, the source stocks are sampled from stocks not listed in the S\&P500 Index (and the target stocks are still sampled from S\&P500 components).

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/score_sp500.png}
         \caption{Risk for cross-sector transfer.}
         \label{fig:score_sp500}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/sharpe_sp500.png}
         \caption{Sharpe ratio for cross-sector transfer.}
         \label{fig:sharpe_sp500}
     \end{subfigure}
     \caption{Relative risk and Sharpe ratio for transfer across sectors with S\&P500 stocks.}
     \label{fig:cross_sector_sp500}
\end{figure}

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/score_nonsp500.png}
         \caption{Risk for cross-sector transfer.}
         \label{fig:score_nonsp500}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/sharpe_nonsp500.png}
         \caption{Sharpe ratio for cross-sector transfer.}
         \label{fig:sharpe_nonsp500}
     \end{subfigure}
     \caption{Relative risk and Sharpe ratio for transfer across sectors with non-S\&P500 stocks.}
     \label{fig:cross_sector_nonsp500}
\end{figure}

Table \ref{tab:cross_sector_corr} records the correlation between Sharpe ratios and transfer risks when transferring portfolios from various source sectors to each target sector. Lower correlation implies that the target sector may benefit more from transfer learning and the transferability is better captured by transfer risk. Similar as the setting in Figure \ref{fig:cross_sector_sp500} and Figure \ref{fig:cross_sector_sp500}, Table \ref{tab:sp500_corr} is from the experiments using S\&P500 source stocks, while Table \ref{tab:nonsp500_corr} is from the experiments using non-S\&P500 source stocks.

\begin{table}[H]
    \begin{subtable}[H]{0.45\textwidth}
        \centering
        \begin{tabular}{cc}
            \toprule
            \toprule
            \textbf{Target Sector} & \textbf{Correlation} \\
            \midrule
            \textbf{Health Care} & -0.88 \\
            \textbf{Communication} & -0.82 \\
            \textbf{Materials} & -0.78 \\
            \textbf{IT} & -0.71 \\
            \textbf{Financials} & -0.60 \\
            \textbf{Consumer} & -0.56 \\
            \textbf{Industrials} & -0.54 \\
            \textbf{Real Estate} & -0.37 \\
            \textbf{Utilities} & -0.20 \\
            \textbf{Energy} & 0.04 \\
            \bottomrule
            \bottomrule
        \end{tabular}
       \caption{S\&P500 stocks.}
       \label{tab:sp500_corr}
    \end{subtable}
    \hfill
    \begin{subtable}[H]{0.45\textwidth}
        \centering
        \begin{tabular}{cc}
            \toprule
            \toprule
            \textbf{Target Sector} & \textbf{Correlation} \\
            \midrule
            \textbf{IT} & -0.67 \\
            \textbf{Materials} & -0.49 \\
            \textbf{Health Care} & -0.47 \\
            \textbf{Communication} & -0.46 \\
            \textbf{Energy} & -0.40 \\
            \textbf{Industrials} & -0.30 \\
            \textbf{Consumer} & -0.28 \\
            \textbf{Real Estate} & -0.14 \\
            \textbf{Financials} & 0.10 \\
            \textbf{Utilities} & 0.17 \\
            \bottomrule
            \bottomrule
        \end{tabular}
        \caption{Non-S\&P500 stocks.}
        \label{tab:nonsp500_corr}
     \end{subtable}
     \caption{Correlation between risk and Sharpe ratio for transfer from other sectors to the target.}
     \label{tab:cross_sector_corr}
\end{table}

Several insightful patterns are observed from above. For sectors such as Health Care and Information Technology, large negative correlations are revealed in Table \ref{tab:cross_sector_corr}, no matter whether the stocks are chosen from S\&P500 or not. This implies that the transfer score appropriately encodes the statistical property and characterizes the transferability of portfolios in those sectors. On the contrary, for sectors such as Utilities and Real Estate, the correlations shown in Table \ref{tab:cross_sector_corr} are not significant, regardless of whether the stocks are chosen from S\&P500 or not. This may result from the fact that companies in Utilities and Real Estate sectors tend to be affected by underlying spatial factors and also changes in regulatory policies. Those aspects may not be fully captured by the transfer risk. In addition, for Energy sector, the correlation is more significant when considering non-S\&P500 stocks. This may due to the industry concentration of Energy sector in S\&P500 Index: Energy sector in S\&P500 Index is highly concentrated to a few large companies, and the portfolio's performance is largely driven by some company-specific factors which the transfer risk fails to capture. The effect of industry concentration dwindles when non-S\&P500 stocks are considered.

\paragraph{Cross-Frequency Transfer.} In the following numerical experiments, we focus on transfer learning between different trading frequencies, ranging from mid-frequency to low-frequency: 1-minute, 5-minute, 10-minute, 30-minute, 65-minute, 130-minute and 1-day.

Given a source frequency and a target frequency, we first randomly sample ten stocks ($d=10$) from the fifty largest US companies by market capitalization. Then, three data sets will be constructed accordingly:

\begin{enumerate}
    \item \textbf{Source training data}: it consists of the returns of ten stocks, sampled under a given source frequency, from February 2016 to September 2019.

    \item \textbf{Target training data}: it consists of the returns of ten stocks, sampled under a given target frequency, from February 2016 to September 2019.

    \item \textbf{Target testing data}: it consists of the returns of ten stocks, sampled under a given target frequency, from September 2019 to February 2020.
\end{enumerate}

The transfer learning scheme applied in the experiments is the same as before: the portfolio is first pre-trained by solving \eqref{eqn:portfolio_opt_source} with the mean and covariance estimated from the source-frequency training data, then fine-tuned by solving \eqref{eqn:portfolio_opt_target} with the mean and covariance estimated from the target-frequency training data. Meanwhile, following the usual setting in mid/high-frequency trading, we assume that over-night holding is not allowed for trading frequencies ranging from 1-minute to 130-minute. More specifically, when over-night holding not is allowed, the price movement after the market close and before the market open will not be included in the mean and covariance estimation. Finally, the performance of the portfolio is evaluated through its Sharpe ratio on the target-frequency testing data. The regularization parameter $\lambda$ in \eqref{eqn:portfolio_opt_target} is set to be $0.2$. Meanwhile, the computation of transfer risk follows the approach described in Section \ref{subsec:port_opt_setup}, using the source-frequency training data and target-frequency testing data. 

For each source-target frequency pair (in total $7\times17=49$ pairs), two hundred random experiments with different stock selections are conducted, and we record the average Sharpe ratio and average transfer risk of those random experiments. The results are presented in Figure \ref{fig:freq_intraday_130min}, Figure \ref{fig:cross_freq_intraday} and Table \ref{tab:cross_freq_corr}. 
%Similar as before, the term ``score'' in the following figures and tables refers to the negation of the transfer score.

For example, Figure \ref{fig:freq_intraday_130min} shows the relation between (average) Sharpe ratios and (average) transfer risks when transferring portfolios from various source frequencies to the target frequency of 130-minute. In general, the negative correlation between Sharpe ratios and scores is observed: when the target frequency is fixed (130-minute in this example), transferring a portfolio from a source frequency with lower transfer risk corresponds to a higher Sharpe ratio. In particular, source frequencies such as 130-minute and 65-minute, which are closer to the 130-minute target frequency, are desirable source tasks, while 1-minute or 1-day is less suitable.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/freq_intraday_130min.png}
    \caption{Transfer risk and Sharpe ratio, transferring to 130-minute frequency.}
    \label{fig:freq_intraday_130min}
\end{figure}

To see more clearly the relation between different frequencies, in Figure \ref{fig:cross_freq_intraday}, we plot the heat maps of transfer risks and Sharpe ratios when transferring across all frequencies. Here the transfer risks and Sharpe ratios are again rescaled linearly, so that for each target frequency, the values will range from zero to one. Meanwhile, Table \ref{tab:cross_freq_corr} records the correlation between Sharpe ratios and transfer risks when transferring portfolios from various source frequencies to each target frequency, following the same setting as Figure \ref{fig:cross_freq_intraday}.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/score_intraday.png}
         \caption{Risk for cross-frequency transfer.}
         \label{fig:score_intraday}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/sharpe_intraday.png}
         \caption{Sharpe ratio for cross-frequency transfer.}
         \label{fig:sharpe_intraday}
     \end{subfigure}
     \caption{Relative risk and Sharpe ratio for transfer across frequencies.}
     \label{fig:cross_freq_intraday}
\end{figure}

\begin{table}[H]
    \centering
    \begin{tabular}{cc}
        \toprule
        \toprule
        \textbf{Target Frequency} & \textbf{Correlation} \\
        \midrule
        \textbf{1 min} & -0.59 \\
        \textbf{5 min} & -0.70 \\
        \textbf{10 min} & -0.74 \\
        \textbf{30 min} & -0.59 \\
        \textbf{65 min} & -0.70 \\
        \textbf{130 min} & -0.76 \\
        \textbf{1 Day} & -0.19 \\
        \bottomrule
        \bottomrule
    \end{tabular}
    \caption{Correlation between risk and Sharpe ratio for transfer from other frequency to the target.}
    \label{tab:cross_freq_corr}
\end{table}

From Figure \ref{fig:cross_freq_intraday}, it is observed that the transfer risks from 1-day frequency to other higher frequencies are relatively high, resulting in poor transfer learning performances as well. This demonstrates a natural discrepancy between low-frequency trading and mid/high-frequency trading: mid/high-frequency trading aims to capture intraday stock price movements by not allowing over-night holding, while low-frequency trading intends to capture price movements across trading days. Consequently, the difference between the underlying statistical properties of intraday price movements and cross-day price movements hurts the performance of transferring a low-frequency portfolio to a mid/high-frequency portfolio. 

Meanwhile, for transfer learning inside the mid/high-frequency regime (1-minute to 130-minute), the results in Figure \ref{fig:cross_freq_intraday} reveal that 65-minute and 130-minute are more appropriate candidates for the source frequency, since they lead to much better transfer learning performance, compared to other higher source frequencies. This may due to the fact that under 65-minute and 130-minute frequencies, the mean and covariance estimations are more robust, hence resulting in a robust source portfolio which performs well after fine-tuning.

% Originally introduced and studied in algebraic topology \cite{chen1954iterated, chen1957integration}, the signature has been widely used in rough path theory \cite{lyons2007differential, friz2010multidimensional}, financial applications \cite{lyons2014feature, arribas2018derivatives, lyons2019numerical, kalsi2020optimal}, time series analysis \cite{morrill2020generalised}, and machine learning \cite{yang2015chinese, xie2017learning, li2017lpsnet, bonnier2019deep, kidger2020signatory}. Benefits of the signature transform include: 1) a high degree of flexibility, making it possible to customise the method to specific data sets; 2) theoretical guarantees about signature features; 3) effectiveness on data sets with small sample size, since no learning is involved in the transform. 


